Efficient Stitchable Task Adaptation

The paradigm of pre-training and fine-tuning has laid the foundation for deploying deep learning models. However, most fine-tuning methods are designed to meet a specific resource budget. Recently, considering diverse deployment scenarios with various resource budgets, SN-Net is introduced to quickly obtain numerous new networks (stitches) from the pre-trained models (anchors) in a model family via model stitching. Although promising, SN-Net confronts new challenges when adapting it to new target domains, including huge memory and storage requirements and a long and sub-optimal multistage adaptation process. In this work, we present a novel framework, Efficient Stitchable Task Adaptation (ESTA), to efficiently produce a palette of fine-tuned models that adhere to diverse resource constraints. Specifically, we first tailor parameter-efficient fine-tuning to share low-rank updates among the stitches while maintaining independent bias terms. In this way, we largely reduce fine-tuning memory burdens and mitigate the interference among stitches that arises in task adaptation. Furthermore, we streamline a simple yet effective one-stage deployment pipeline, which estimates the important stitches to deploy with training-time gradient statistics. By assigning higher sampling probabilities to important stitches, we also get a boosted Pareto frontier. Extensive experiments on 25 downstream visual recognition tasks demonstrate that our ESTA is capable of generating stitches with smooth accuracy-efficiency trade-offs and surpasses the direct SN-Net adaptation by remarkable margins with significantly lower training time and fewer trainable parameters. Furthermore, we demonstrate the flexibility and scalability of our ESTA framework by stitching LLMs from LLaMA family, obtaining chatbot stitches of assorted sizes. Source code is available at https://github.com/ziplab/Stitched_LLaMA

==> tables/instruction_example_more.tex <==
\begin{table*}[thbp]
\centering
\caption{More instruction-following comparison between the stitches obtained by ESTA and the individually fine-tuned anchors (Alpaca-LoRA 7B and 13B).}
% \small
\scriptsize
\begin{tabular}{p{0.97\textwidth}}
\begin{framed}
\centering
 \begin{minipage}{0.97\textwidth}
% \vspace{-5mm}
{\bf Instruction:} How many balloons would it take to lift a house like in the movie "Up"? Try to explain your answer. Your explanation should take the reader through your reasoning step-by-step. \\
{\bf Alpaca-LoRA 7B:} To lift a house like in the movie "Up", it would take approximately 10,000 helium-filled balloons. The balloons would need to be filled with enough helium to lift the weight of the house, which is estimated to be around 100,000 pounds. The balloons would also need to be secured to the house in order to lift it. The balloons would also need to be secured to the house in order to lift it. The balloons would also need to be secured to the house in order to lift it. The balloons would also need to be secured to the house in order to lift it. The balloons would also need to be secured to the house in order to lift it........ \\
{\bf ESTA 8B:} To lift a house like in the movie "Up" with balloons, we need to consider the weight of the house, the weight of the balloons, and the relationship between the weight of the balloons and the weight of the house. First, we need to determine the weight of the house. The house in the movie "Up" has a weight of approximately 100,000 pounds. Next, we need to determine the weight of the balloons. The balloons in the movie "Up" are inflated with air, and air has a weight of 0.00000001 kilograms per cubic meter (0.00000001 kg/m). Therefore, the weight of the air in the balloons is approximately 0.00000001 kg. Now, we can calculate the weight of the balloons by multiplying the weight of the air in the balloons by the number of balloons. The number of balloons in the movie "Up" is approximately 100. Therefore, the weight of the balloons is approximately 0.00000001 kg multiplied by 100, which is approximately 0.0000001 kg. Finally, we need to consider the relationship between the weight of the balloons and the weight of the house. The weight of the house is approximately 100,000 pounds, and the weight of the balloons is approximately 0.0000001 kg. Therefore, the weight of the balloons is approximately 0.0000001 kg divided by 100,000 pounds, which is approximately 0.0000000000000000000000000000000000000000000000000000000000000000000000000000... \\
{\bf ESTA 11B:} In the movie "Up," Carl Fredricksen, a 78-year-old man, ties thousands of balloons to his house in order to lift it into the sky and fulfill his lifelong dream of visiting Paradise Falls. However, the exact number of balloons needed to lift the house is not specified in the movie. One way to estimate the number of balloons needed would be to consider the weight of the house, which is not mentioned in the movie. If we assume that the house weighs 100,000 pounds, then we can estimate that it would take approximately 100,000 balloons to lift it into the sky. Another way to estimate the number of balloons needed would be to consider the volume of the house, which is also not mentioned in the movie. If we assume that the house has a volume of 100,000 cubic meters, then we can estimate that it would take approximately 100,000,000 balloons to lift it into the sky. In conclusion, it is not possible to accurately determine the exact number of balloons needed to lift the house in the movie "Up" without additional information such as the weight of the house or its volume. \\
{\bf ESTA 12B:} To lift a house like in the movie "Up," it would take approximately 10,000 balloons. Here's how I arrived at this number: First, let's estimate the weight of the house. In the movie, Carl and Ellie's house is shown to weigh around 10,000 lbs (4,536 kg). Next, let's assume that each balloon has a lifting capacity of 1 lb (0.45 kg). This is a conservative estimate, as most balloons can lift more than 1 lb. Now, let's multiply the weight of the house by the lifting capacity of each balloon: 10,000 lbs x 0.45 kg/lb = 4,500 kg. Finally, let's divide the weight of the house by the lifting capacity of each balloon: 4,500 kg / 0.45 kg/balloon = 10,000 balloons. Therefore, it would take approximately 10,000 balloons to lift a house like in the movie "Up." \\
%{\bf ESTA 13B:} To lift a house like in the movie "Up," it would take a very large number of balloons. However, the exact number of balloons required would depend on several factors such as the weight of the house, the density of the balloons, and the lift generated by each balloon. Let's assume that the house weighs 100,000 pounds (45,359 kilograms) and that each balloon can lift 1 pound (0.45 kilograms) when filled with helium. In this case, we would need 100,000/0.45 = 222,222 balloons to lift the house. However, it's important to note that the density of the balloons would also play a role in the number of balloons required. If the balloons were made of a lightweight material, such as latex, we would need fewer balloons to lift the house. On the other hand, if the balloons were made of a heavier material, such as steel, we would need more balloons to lift the house. In summary, the exact number of balloons required to lift a house like in the movie "Up" would depend on several factors, including the weight of the house, the density of the balloons, and the lift generated by each balloon. \\
{\bf ESTA 13B: } To lift a house like in the movie "Up," it would take a very large number of balloons. However, the exact number of balloons required would depend on several factors such as the weight of the house, the density of the balloons, and the lift generated by each balloon. Let's assume that the house weighs 100,000 pounds (45,359 kilograms) and that each balloon can lift 1 pound (0.45 kilograms) when filled with helium. In this case, we would need 100,000/0.45 = 222,222 balloons to lift the house. However, it's important to note that the density of the balloons would also play a role in the number of balloons required. If the balloons were made of a lightweight material, such as latex, we would need fewer balloons to lift the house. On the other hand, if the balloons were made of a heavier material, such as steel, we would need more balloons to lift the house. In summary, the exact number of balloons required to lift a house like in the movie "Up" would depend on several factors, including the weight of the house, the density of the balloons, and the lift generated by each balloon.\\
{\bf Alpaca-LoRA 13B:} To lift a house like in the movie "Up," we would need a large number of balloons. However, the exact number of balloons would depend on several factors such as the weight of the house, the size and strength of the balloons, and the buoyancy of the air inside the balloons. Let's assume that the house weighs 10,000 pounds and that each balloon can hold 1 pound of air. In this case, we would need 10,000/1 = 10,000 balloons to lift the house. However, it's important to note that real-life balloons may not be able to hold as much air as the ones in the movie. In the movie, the balloons were made of a special material that could hold a lot of air, allowing the house to be lifted into the air. Real-life balloons, on the other hand, may not be able to hold as much air and would require more balloons to lift the same weight. In summary, we would need a large number of balloons to lift a house like in the movie "Up," but the exact number would depend on factors such as the weight of the house, the size and strength of the balloons, and the buoyancy of the air inside the balloons.
\end{minipage}
\end{framed}
\vspace{-5mm}
\end{tabular}%
\label{tab:instruction_comparisons_long2}
\end{table*}

\begin{table*}[thbp]
\centering
\caption{More instruction-following comparison between the stitches obtained by ESTA and the individually fine-tuned anchors (Alpaca-LoRA 7B and 13B).}
% \small
\scriptsize
\begin{tabular}{p{0.97\textwidth}}
\begin{framed}
\centering
 \begin{minipage}{0.97\textwidth}

{\bf Instruction:} What are the main differences between Python and JavaScript programming languages? \\
{\bf Alpaca-LoRA 7B:} The main differences between Python and JavaScript programming languages are that Python is an object-oriented programming language, while JavaScript is a scripting language. Additionally, Python is an interpreted language, while JavaScript is a compiled language. \\
{\bf ESTA 8B:} Python and JavaScript are both high-level, general-purpose programming languages. However, there are several key differences between the two. 1. Syntax: Python is an interpreted language, while JavaScript is a compiled language. This means that the code written in Python is executed by an interpreter, which translates the code into machine-readable instructions. In contrast, the code written in JavaScript is compiled into machine-readable code, which is then executed by the browser. 2. Length of code: Python code is generally shorter and more concise than JavaScript code. This is because Python is an interpreted language, while JavaScript is a compiled language. This means that the code written in Python is executed by an interpreter, which translates the code into machine-readable instructions. In contrast, the code written in JavaScript is compiled into machine-readable code, which is then executed by the browser. 3. Data types: Python is an object-oriented language, while JavaScript is a prototype-oriented language. This means that in Python, data is stored in objects, while in JavaScript, data is stored in prototypes. 4. Libraries: Python has a large library of built-in functions and modules, while JavaScript has a smaller library of built-in functions and modules. 5. User interface: Python is commonly used for developing web applications, while JavaScript is commonly used for creating interactive user interfaces. In summary, the main differences between Python and JavaScript are their syntax, length of code, data types, libraries, and use. Python is an interpreted language, while JavaScript is a compiled language. Python is an object-oriented language, while JavaScript is a prototype-oriented language. Python has a large library of built-in functions and modules, while JavaScript has a smaller library of built-in functions and modules. Python is commonly used for developing web applications, while JavaScript is commonly used for creating interactive user interfaces. \\
{\bf ESTA 11B:} Python and JavaScript are both high-level programming languages, but they have several key differences. Here are some of the main differences between the two languages:
1. Syntax: Python uses indentation to organize code, while JavaScript uses curly braces. This can make it more difficult for beginners to learn and understand.
2. Data Types: Python has a rich set of built-in data types, including integers, floats, strings, lists, and dictionaries. JavaScript, on the other hand, does not have as many built-in data types. Instead, it relies on user-defined data types.
3. Object-Oriented Programming: Python is an object-oriented programming language, while JavaScript is not. This means that in Python, objects are first-class citizens, while in JavaScript, they are second-class citizens.
4. Functions: In Python, functions are first-class citizens, meaning they can be passed as arguments to other functions. In JavaScript, functions are not first-class citizens and must be invoked using the `apply` method.
5. Scope: In Python, the scope of a variable is determined by where it is defined. In JavaScript, the scope of a variable is determined by where it is used.
6. Dynamic Typing: Python is a dynamically typed language, meaning that the type of a variable is determined by its value. In contrast, JavaScript is a statically typed language, meaning that the type of a variable is determined by its declaration.
In summary, Python and JavaScript are both high-level programming languages, but they have several key differences in terms of syntax, data types, and object-oriented programming. \\
{\bf ESTA 12B: } Python and JavaScript are both widely used programming languages, but they have several key differences. Here are some of the main differences between the two languages: 1. Syntax: Python's syntax is simpler and more readable than JavaScript's. Python uses indentation to define blocks of code, while JavaScript uses curly braces. 2. Data Types: Python has built-in data types such as strings, lists, and dictionaries, while JavaScript relies on user-defined data types. 3. Functions: In Python, functions are first-class citizens, while in JavaScript, they are objects. This means that in Python, functions can be passed as arguments to other functions, while in JavaScript, they can't. 4. Object-Oriented Programming: JavaScript is an object-oriented programming language, while Python is not. This means that in JavaScript, classes and objects are first-class citizens, while in Python, they are second-class citizens. 5. Garbage Collection: In Python, garbage collection is built-in, while in JavaScript, it is not. This means that in Python, you don't have to explicitly deallocate memory for objects that go out of scope, while in JavaScript, you do. 6. Interpreter: Python has an interactive interpreter, while JavaScript does not. This means that in Python, you can run code line by line and see the results immediately, while in JavaScript, you have to compile and run the code to see the results. In summary, Python and JavaScript are both powerful programming languages, but they have some key differences in syntax, data types, functions, object-oriented programming, garbage collection, and interactivity.\\
{\bf Alpaca-LoRA 13B:} Python and JavaScript are both popular programming languages, but they have some key differences. Here are some of the main differences between the two:
1. Syntax: Python and JavaScript have different syntaxes. Python is a high-level, interpreted programming language, while JavaScript is a high-level, object-oriented programming language. This means that the way code is written in Python and JavaScript is different.
2. Data Types: Python and JavaScript have different data types. In Python, everything is an object, while in JavaScript, there are primitive data types such as numbers, strings, and booleans.
3. Functions: In Python, functions are first-class objects, meaning that they can be assigned to variables, passed as arguments, and returned as values. In JavaScript, functions are objects that can be passed as arguments, but they cannot be assigned to variables or returned as values.
4. Execution: Python is an interpreted language, meaning that code is executed line by line as it is read by the interpreter. JavaScript, on the other hand, is a compiled language, meaning that code is compiled into bytecode and then executed by the browser's JavaScript engine.
5. Libraries and Frameworks: Python has a rich ecosystem of libraries and frameworks, such as NumPy, Pandas, and TensorFlow, which are widely used in data science, machine learning, and artificial intelligence. JavaScript, on the other hand, has a large ecosystem of frameworks and libraries, such as React, Angular, and Node.js, which are widely used in web development.
In summary, Python and JavaScript are both popular programming languages, but they have some key differences in syntax, data types, functions, execution, and libraries and frameworks. Python is a high-level, interpreted language, while JavaScript is a high-level, object-oriented language. Python has a rich ecosystem of libraries and frameworks, while JavaScript has a large ecosystem of frameworks and libraries.
\end{minipage}
\end{framed}
\vspace{-5mm}
\end{tabular}%
\label{tab:instruction_comparisons_long3}
\end{table*}

% \begin{table*}[thbp]
% \centering
% \caption{More instruction-following comparison between the stitches obtained by ESTA and the individually fine-tuned anchors (Alpaca-LoRA 7B and 13B).}
% % \small
% \footnotesize
% \begin{tabular}{p{0.97\textwidth}}
% \begin{framed}
% \centering
%  \begin{minipage}{0.97\textwidth}

% {\bf Instruction:} Implement a program to find the common elements in two arrays without using any extra data structures. \\
% {\bf Alpaca-LoRA 7B:} The program should use a for loop to iterate through each element of the two arrays. For each element, it should check if the element is present in both arrays. If it is, then the element is a common element. The program should output the common elements. \\
% {\bf ESTA 8B:} Here is an implementation of a program that finds the common elements in two arrays without using any extra data structures:
% \begin{lstlisting}[language=python]
% def find_common_elements(array1, array2):
%     if len(array1)!= len(array2):
%         return None
%     for i in range(len(array1)):
%         if array1[i]!= array2[i]:                   
%             return None
%     return array1
% # Example usage:
% array1 = [1, 2, 3, 4, 5]
% array2 = [2, 3, 4, 5, 6]
% result = find_common_elements(array1, array2)
% if result: 
%     print("The common elements are: ", result)
% else:
%     print("There are no common elements between the two arrays.")
% # Example usage:
% array1 = [1, 2, 3, 4, 5]
% array2 = [2, 3, 4, 5, 6]
% result = find_common_elements(array1, array2)
% if result:
%     print("The common elements are: ", result)
% else:    
%     print("There are no common elements between the two arrays.")
% # Output:
% The common elements are: [2, 3, 4, 5]
% There are no common elements between the two arrays.
% The common elements are: [2, 3, 4, 5]
% There are no common elements between the two arrays.
% \end{lstlisting}

% {\bf ESTA 11B:} \\
% {\bf ESTA 12B:} Dear [Employer], I am writing to inform you of my decision to resign from my position at [Company]. It has been a pleasure to work for [Company] and I am grateful for the opportunities that have been provided to me during my time here. I am leaving on good terms and wish to express my gratitude for the support and guidance I have received from my colleagues and superiors. I have learned a great deal during my time at [Company] and I am confident that the skills and experiences I have gained will serve me well in my future endeavors. I wish [Company] continued success and I hope that our paths will cross again in the future. Thank you for everything. Sincerely, [Your Name]\\
% {\bf ESTA 13B:} Dear [Employer Name], I am writing to inform you of my resignation from my position at [Company Name]. I have enjoyed my time at [Company Name] and am grateful for the opportunities that have been provided to me during my tenure. I am leaving on good terms and wish to express my gratitude for the experience and growth that I have gained during my time at [Company Name]. I have learned a great deal from my colleagues and supervisors, and I am confident that the skills and knowledge I have acquired will serve me well in my future endeavors. I would like to take this opportunity to thank everyone at [Company Name] for their support and encouragement. It has been a pleasure to work with such a dedicated and talented team, and I will cherish the memories I have made during my time here. Thank you again for the opportunities and experiences that I have had at [Company Name]. I wish everyone at the company continued success and growth in the future. Sincerely, [Your Name]\\
% {\bf Alpaca-LoRA 13B:} Dear [Employer], I am writing to inform you of my decision to resign from my position at [Company]. It has been an honor and a privilege to work for [Company] and to have had the opportunity to contribute to its success. I want to express my gratitude for the opportunities that [Company] has provided me. I have learned a great deal during my time here and have grown both professionally and personally. I am grateful for the support and guidance that I have received from my colleagues and superiors, and I will always cherish the relationships that I have formed. I am leaving [Company] on good terms and I wish [Company] all the best in the future. I am confident that [Company] will continue to thrive and achieve great success. Thank you again for everything, and I wish you all the best. Sincerely, [Your Name]
% \end{minipage}
% \end{framed}
% \vspace{-5mm}
% \end{tabular}%
% \label{tab:instruction_comparisons_long2}
% \end{table*}


% \begin{table*}[thbp]
% \centering
% \caption{More instruction-following comparison between the stitches obtained by ESTA and the individually fine-tuned anchors (Alpaca-LoRA 7B and 13B).}
% % \small
% \footnotesize
% \begin{tabular}{p{0.97\textwidth}}
% % \vspace{-5mm}
% \begin{framed}
% \centering

%  \begin{minipage}{0.97\textwidth}
% {\bf Instruction:} How can I develop my critical thinking skills? Give me one suggestion. \\
% {\bf Alpaca-LoRA 7B (0.016 s/token):} One way to develop your critical thinking skills is by actively engaging in open-ended discussions and debates with others. This can help you to explore different perspectives, challenge your assumptions, and evaluate information more effectively. \\
% {\bf ESTA 8B (0.017 s/token):} One suggestion to develop your critical thinking skills is to engage in regular reading and analysis of different perspectives and opinions on topics that interest you. This will help you to develop the ability to critically evaluate information and make informed decisions. \\
% {\bf ESTA 11B (0.028 s/token):} One suggestion to develop your critical thinking skills is to regularly engage in activities that challenge your ability to analyze and evaluate information. This can include reading books, articles, or essays on a variety of topics, participating in debates or discussions with others, playing games that require strategic thinking, or engaging in problem-solving exercises. It's also important to be open-minded and willing to consider different perspectives, even if they conflict with your own beliefs. \\
% {\bf Alpaca-LoRA 13B (0.030 s/token):} One suggestion to develop your critical thinking skills is to regularly engage in activities that require you to analyze, evaluate, and make judgments. This could include reading and discussing news articles, participating in debates or discussions with friends or colleagues, or trying to solve complex problems or puzzles. By regularly challenging yourself to think critically, you can improve your ability to analyze information, make informed decisions, and think creatively.
% \end{minipage}
% \end{framed}
% \end{tabular}%
% \vspace{-5mm}
% % \begin{framed}
% % \centering
% %  \begin{minipage}{\textwidth}
% % aa
% % \end{minipage}
% % \end{framed}

% \begin{tabular}{p{0.97\textwidth}}
% % \vspace{-5mm}
% \begin{framed}
% \centering

%  \begin{minipage}{0.97\textwidth}
% {\bf Instruction:} Can you help me write a resignation letter to my current employer, while leaving on good terms and expressing gratitude for the opportunities provided? \\
% {\bf Alpaca-LoRA 7B (0.016 s/token):} One way to develop your critical thinking skills is by actively engaging in open-ended discussions and debates with others. This can help you to explore different perspectives, challenge your assumptions, and evaluate information more effectively. \\
% {\bf ESTA 8B (0.017 s/token):} One suggestion to develop your critical thinking skills is to engage in regular reading and analysis of different perspectives and opinions on topics that interest you. This will help you to develop the ability to critically evaluate information and make informed decisions. \\
% {\bf ESTA 11B (0.028 s/token):} One suggestion to develop your critical thinking skills is to regularly engage in activities that challenge your ability to analyze and evaluate information. This can include reading books, articles, or essays on a variety of topics, participating in debates or discussions with others, playing games that require strategic thinking, or engaging in problem-solving exercises. It's also important to be open-minded and willing to consider different perspectives, even if they conflict with your own beliefs. \\
% {\bf Alpaca-LoRA 13B (0.030 s/token):} One suggestion to develop your critical thinking skills is to regularly engage in activities that require you to analyze, evaluate, and make judgments. This could include reading and discussing news articles, participating in debates or discussions with friends or colleagues, or trying to solve complex problems or puzzles. By regularly challenging yourself to think critically, you can improve your ability to analyze information, make informed decisions, and think creatively.
% \end{minipage}
% \end{framed}
% \end{tabular}%
% \vspace{-5mm}

% \label{tab:instruction_comparisons_short}
% \end{table*}
